Variational Inference with Normalizing Flows

The choice of approximate posterior distribution is one of the core problems in variational inference. Most applications of variational inference employ simple families of posterior approximations in order to allow for efficient inference, focusing on mean-field or other simple structured approximations. This restriction has a significant impact on the quality of inferences made using variational methods. We introduce a new approach for specifying flexible, arbitrarily complex and scalable approximate posterior distributions. Our approximations are distributions constructed through a normalizing flow, whereby a simple initial density is transformed into a more complex one by applying a sequence of invertible transformations until a desired level of complexity is attained. We use this view of normalizing flows to develop categories of finite and infinitesimal flows and provide a unified view of approaches for constructing rich posterior approximations. We demonstrate that the theoretical advantages of having posteriors that better match the true posterior, combined with the scalability of amortized variational approaches, provides a clear improvement in performance and applicability of variational inference.

==> algo.tex <==
\section {VAEs / DLGMs \label{sec:DLGM}}

VAEs/DLGMs are directed generative models $p_{\theta} ( \vx |\vz ) p(\vz)$ with latent variables $\vz$, where the prior over the latents is a unit Gaussian $p(\vz) = \N(\vzero, \vI)$ and the observation likelihood $p_{\theta} ( \vx |\vz )$ is a simple distribution conditioned on $\vz$ that is parametrized by a MLP as illustrated in figure \ref{fig:archs}.

For these models, we introduce a fixed-form inference density $q_{\phi} (\vz | \vx)$ with parameters $\vphi$ that approximates the true posterior distribution $p_{\theta}(\vz | \vx)$. This is a widely used approach to variational inference \citep{kingma2014stochastic, rezende2014stochastic, Dayan2000, stuhlmuller2013learning}. 

Using an inference network, we avoid the need to compute per data point variational parameters, but can instead compute a set of global variational parameters $\vphi$ valid for both training and test data. This allows us to amortize the cost of inference by generalizing between the posterior estimates for all latent variables through the parameters of the inference network. The simplest inference models that we can use are diagonal Gaussian densities, 
\begin{align}
q_{\phi} (\vz  | \vx) &= \N(\vz | \vmu_{\phi}(\vx), \diag(\vsigma_{\phi}^2(\vx)) ), \label{eq:recogModel1}
\end{align}
where the mean function $\vmu_{\phi}(\vx)$ and the standard-deviation function $\vsigma_{\phi}(\vx)$ are represented as MLPs.

Learning is performed by minimizing the variational bound in equation \eqref{eq:FE} resulting from the introduction of an approximate inference network $q_{\phi} ( \vz | \vx )$ that is also parametrized by a MLP. 
The inference networks used in \cite{kingma2014stochastic, rezende2014stochastic} are simple diagonal or diagonal+low-rank Gaussian densities. The gradients of the variational bound  \eqref{eq:FE} are approximated using the "reparametrization trick" briefly explained below.


\section{Simple families of flows}

It is straight-forward to build invertible MLPs that could be used in equation \eqref{eq:drule}, \cite{baird2005one}. However, the algorithmic complexity of computing the det-Jacobian terms in \eqref{eq:drule} will scale as $O(K d^3)$ where $d$ is the dimension of the layers and $K$ is the number of layers. Moreover, computing the gradients of the det-Jacobian terms involves several additional operations which are also $O(K d^3)$ and are numerically tricky, involving matrix inverses.
Therefore it is important to find architectures for which the det-Jacobian terms are either cheap to compute or are not needed at all, \cite{dinh2014nice}.

Here we introduce and compare different families of flows. In section \ref{sec:results} we analyze their impact on learned VAEs for different datasets.

\subsection{ Deep MLPs with a single neuron per layer }

This model consists of a family of transformations the form 
\begin{align}
  f ( \vz ) &=\vz+\vu h ( \vw^{T} \vz+b ),  \label{eq:map}
\end{align}
where $\vz, \vw, \vu \in \Reals^{d}  , b \in \Reals$ and $h ( \bullet )$ is
any smooth element-wise non-linearity has been introduced and analyzed.

For this simple map we can compute the log-det-Jacobian term in $O(d)$ time (using the matrix determinant lemma):
\begin{align}
  \left| \det   \frac{\partial f}{\partial \vz} \right| &= | \det (
  \vI+\vu \psi ( \vz )^{T} ) | = | 1+\vu^{T} \psi ( \vz ) |  
\end{align}
where
\begin{align}
  \psi ( \vz ) &= h' ( \vw^{T} \vz+b ) \vw.
\end{align}
From \eqref{eq:nested} we conclude that the density $q_{K} ( \vz )$ obtained by transforming an arbitrary initial density $q_0(\vz)$ through the sequence of maps $f_{k} ,k=1 \ldots K$ with parameters
$\{ \vu_{k} \in \Reals^{d} , \vw_{k} \in \Reals^{d} ,b_{k} \in
\Reals \}$ is implicitly given by
\begin{align}
  \ln  q_{K} ( f_{K} \circ f_{K-1} \circ   \ldots   \circ  f_{1} ( \vz ) ) &=
  \ln  q_{0} ( \vz ) \nonumber\\
   &- \sum_{k=1}^{K} \ln | 1+\vu_{k}^{T} \psi_{k} ( \vz_{k} ) |. \label{eq:nested_maps}
\end{align}
Functions of the form \eqref{eq:map} are not always invertible depending on the non-linearity and parameters chosen. If $h(x) = \text{tanh}(x)$ we have that a sufficient condition for $f(\vz)$ being invertible is that $\vw^T \vu > -1$.
We enforce this constraint by taking an arbitrary vector $\vu$ and modifying its component parallel to $\vw$, producing a new vector $\hat{\vu}$ such that $\vw^T \hat{\vu} > -1$. The modified vector can be compactly written as $\hat{\vu}(\vw, \vu) = \vu + \left [ r(\vw^T\vu) - (\vw^T\vu) \right] \frac{\vw}{|| \vw ||^2}$, where the scalar function $r(x)$ is given by $r(x) = -1 + \log (1 + e^x)$.

Additionally, when the element-wise function $h$ is the identity-function, this flow corresponds to adding $K$ rank-one corrections to the covariance matrix of $q_0$. 

\subsection{NICE}

In \cite{dinh2014nice} a family of invertible, volume-preserving neural nets has been proposed. They are of the form
\begin{align}
  f ( \vz ) &=( \vz_A, \vz_B + h_{\theta} ( \vz_A ) ),  \label{eq:nice_map}
\end{align}
where $\vz = (\vz_A, \vz_B)$ is an arbitrary partitioning of the vector $\vz$ and $h_{\theta}$ is an arbitrary smooth function parametrized by a MLP.
These maps can be trivially inverted
\begin{align}
g(\vz') &= ( \vz'_A, \vz'_B - h_{\theta} ( \vz'_A ) ). \label{eq:nice_map_inverse}
\end{align}
In order to build a flow capable of mixing all components of the initial vector $\vz_0\sim q_{0}$ such flows must alternate between different partitionings of $\vz_k$. The resulting density is given by a simple expression 
\begin{align}
  \ln  q_{K} ( f_{K} \circ f_{K-1} \circ   \ldots   \circ  f_{1} ( \vz_0 ) ) &=
  \ln  q_{0} ( \vz_0 ). \label{eq:nested_maps_nice}
\end{align}
Since the inverse flow is also known, we can express the density $q_{K}$ directly as 
\begin{align}
  \ln  q_{K} (\vz') &= q_0( g_{1} \circ g_{2} \circ   \ldots   \circ  g_{K} ( \vz' ) ). \label{eq:nested_maps_nice_inverse}
\end{align}

We compare two mechanisms for mixing the components of $\vz$ before separating them in two disjoint subgroups $\vz_A$ and $\vz_B$. 

The first mechanism consists in applying a random permutation. 
The second consists in applying a random orthogonal transformation
\footnote{ Random orthogonal transformations can be generated by sampling a matrix with independent unit-Gaussian entries $A_{i,j} \sim \mathcal{N}(\vzero,\vI)$ and then performing a QR-factorization. The resulting $Q$-matrix will be a random orthogonal matrix \cite{genz1998methods}.}.

\begin{figure}[ht]
\centering
\subfigure[Inference model using \eqref{eq:nested_maps}]{%
\includegraphics[width=3.6cm]{figures/archs_inference_simple.pdf}
\label{fig:arch_inference_simple}}
\quad
\subfigure[Inference model using \eqref{eq:nested_maps_nice}]{%
\includegraphics[width=3.6cm]{figures/archs_inference_nice.pdf}
\label{fig:arch_inference_nice}}
\quad
%
\caption{Inference networks where two Maxout layers map the observations to the parameters of the flow. Round containers represent layers of stochastic variables whereas square containers represent deterministic layers.}
\label{fig:arch_inference}
\end{figure}

\section{Reparametrized bound \label{sec:rep_bound}}

We can now construct a very flexible conditional posterior density $q ( \vz | \vx )$ by building a neural network that maps the observation $\vx$ to the parameters of the flow $f_{k= 1 \ldots K}$ and the parameters of the initial density $q_0$. 
The specific neural architectures used in this paper are illustrated in figure \ref{fig:arch_inference}.

If we parametrize the inference model as $q_{\phi}( \vz | \vx ) := q_{K} ( \vz_{K} )$ the bound \eqref{eq:FE} can be written as an expectation over the initial distribution $q_0(\vz)$
\begin{align}
  \FE(\vx) & = \E_{q_{\phi} ( \vz | \vx )} [ \log  q_{\phi} ( \vz | \vx ) - \log  p ( \vx, \vz ) ] \nonumber \\
  &= \E_{q_{0} ( \vz_0 )} \left [ \ln  q_{K} ( f_{K} \circ f_{K-1} \circ  
  \ldots   \circ  f_{1} ( \vz_0 ) ) \right . \nonumber \\
   & \left. - \log  p ( \vx ,f_{K} \circ f_{K-1}
  \circ   \ldots   \circ  f_{1} ( \vz_0 ) ) \right ] \nonumber \\
  %&= -H[\vz_0] - \E_{q_{0} ( \vz_0 )} \left [ \log  p ( \vx  , f_{K} \circ f_{K-1}
  %  \circ   \ldots   \circ  f_{1} ( \vz_0 ) ) \right] \nonumber \\
  &= \E_{q_{0} ( \vz_0 )} \left[ \ln  q_{0} ( \vz_0 ) \right] \nonumber \\ 
  &- \E_{q_{0} ( \vz_0 )} \left[ \sum_{k=1}^{K} \ln |
  1+u_{k}^{T} \psi_{k} ( \vz_{k} ) | \right] \nonumber \\ 
  &- \E_{q_{0} ( \vz_0 )} \left[\log  p ( \vx ,f_{K} \circ
  f_{K-1} \circ   \ldots   \circ  f_{1} ( \vz_0 ) ) \right]. \label{eq:tbound}
\end{align}


\section{Optimization}
\label{sect:infer_optim}

The bound in equations \eqref{eq:FE} provide a unified objective function for optimization of both the parameters $\vtheta$ and $\vphi$ of the generative and inference models, respectively. Its minimization can be done jointly by using deterministic reparametrization of the expectations combined with Monte Carlo approximation. This is referred to in previous work as \emph{stochastic gradient variational Bayes} (SGVB) \citep{kingma2014stochastic} or as \emph{stochastic backpropagation} \citep{rezende2014stochastic}.  

When the prior $p(\vz)$ is a spherical Gaussian distribution $p(\vz) = \mathcal{N}(\vz| \vzero, \vI)$ and the variational distribution $q_{\phi} (\vz|\vx)$ is also a Gaussian distribution, the KL term in equation \eqref{eq:FE} can be computed analytically and the log-likelihood term can be rewritten, using the location-scale transformation for the Gaussian distribution, as:
\begin{align}
 \expect{q_{\phi} (\vz|\vx) } { \log p_{\theta}(\vx | \vz) }  &=  \E_{ \mathcal{N}( \vepsilon | \vzero, \vI ) } [ \log p_{\theta}(\vx |  \vmu_{\phi}(\vx)] \nonumber \\
 &+ \E_{ \mathcal{N}( \vepsilon | \vzero, \vI ) } [ \vsigma_{\phi}(\vx) \odot \vepsilon ) ], \label{eq:reparametrization}
\end{align}
where $\odot$ indicates the element-wise product.
While the expectation \eqref{eq:reparametrization} still cannot be solved analytically, its gradients with respect to the generative parameters  $\vtheta$ and  variational parameters $\vphi$ can be efficiently computed as expectations of simple gradients:
\begin{align}
\nabla_{ \{\theta, \phi\} } \E_{q_{\small \phi} }[\log p_{\theta}(\vx | \vz) ] &=  \E_{ \mathcal{N}( \vepsilon | \vzero, \vI )  } [ \nabla_{ \{\theta, \phi\} } \log p_{\theta}(\vx |  \vmu_{\phi}(\vx) ] \nonumber \\
 &+ \E_{ \mathcal{N}( \vepsilon | \vzero, \vI )  } [ \vsigma_{\phi}(\vx) \odot \vepsilon)   ]. \label{eq:reparametrizationGradThetaPhi}
\end{align}

The estimated gradients are used in conjunction with standard stochastic gradient-based optimization methods such as RMSprop or AdaGrad~\citep{duchi2010adaptive}.
This results in parameter updates of the form: $
(\vtheta^{t+1}, \vphi^{t+1}) \gets (\vtheta^{t}, \vphi^{t}) + \boldsymbol{\Gamma}^t (\vg^t_{\theta}, \vg^t_{\phi} ), \nonumber
$
where $\vGamma$ is a diagonal preconditioning matrix that adaptively scales the gradients for faster minimization.

\subsection{Algorithm Summary and Complexity}

The resulting algorithm is a simple modification  of \cite{kingma2014stochastic, rezende2014stochastic}, which we summarize in algorithm \ref{alg:VAENF}.

The algorithmic complexity of computing the gradient through a flow of length $K$ is $O(K d)$, where $d$ is the dimension of the latent variables.

\begin{algorithm}[h!]
\caption{VAE with Normalizing Flow}
\begin{algorithmic}
\STATE{Parameters: $\vphi $ variational, $\vtheta$ generative}
\WHILE{not converged}
    \STATE{$\vx \leftarrow $} \COMMENT{Get mini-batch}
    \STATE{$\vz_0 \sim q_0(\bullet | \vx)$}
    \STATE{$\vz_K \leftarrow f_{K} \circ f_{K-1} \circ   \ldots   \circ  f_{1} ( \vz_0 )$}
    \STATE{$\J(\vx) \approx \J(\vx,\vz_K)$}
	\STATE{$\Delta \vtheta \propto -\nabla_{\theta} \J(\vx)$}
	\STATE{$\Delta \vphi \propto -\nabla_{\phi} \J(\vx)$}
\ENDWHILE
\end{algorithmic}
\label{alg:VAENF}
\end{algorithm}
